Refined Grey-Box Fuzzing with SIVO

We design and implement from scratch a new fuzzer called SIVO that refines multiple stages of grey-box fuzzing. First, SIVO refines data-flow fuzzing in two ways: (a) it provides a new taint inference engine that requires only logarithmic in the input size number of tests to infer the dependency of all program branches on the input bytes, and (b) it deploys a novel method for inverting branches by solving directly and efficiently systems of inequalities. Second, our fuzzer refines accurate tracking and detection of code coverage with simple and easily implementable methods. Finally, SIVO refines selection of parameters and strategies by parameterizing all stages of fuzzing and then dynamically selecting optimal values during fuzzing. Thus the fuzzer can easily adapt to a target program and rapidly increase coverage. We compare our fuzzer to 11 other state-of-the-art grey-box fuzzers on 27 popular benchmarks. Our evaluation shows that SIVO scores the highest both in terms of code coverage and in terms of number of found vulnerabilities.

==> chapters/minor.tex <==
% !TEX root = ../paper.tex

\section{The Gray-box fuzzer \fazer }

\subsection{Additional Advances}
\label{sec:minor}

\begin{itemize}


  
\item \textbf{Accurate code coverage.} We make two improvements to the AFL's code coverage. 
First, to measure multiplicity of an edge, AFL uses byte counter\footnote{Increasing the size of the counter is suboptimal as the new array may not fit in the L1 cache.}, which sometimes overflows, and hence leads to incorrect coverage information (e.g. edge seen 256 times is reported as not visited). We prevent such overflows by limiting the counters to 255. 
Second, we prevent colliding edges, problem addressed and supposedly solved by CollAFL~\cite{}, using much simpler method. (CollAFL solution code is not available; from our analysis it seems that implementing the solution is not universally supported by the current LLVM, but requires ad-hoc change to the installation scripts of the binaries). 
More precisely, in line with Bloom filters, we use two hash functions (instead of only one) to decide the positions of the counter increase. Our analysis given in Appendix XXX, shows significant reduction in the collision probabilities. 
 
  
\item \textbf{Utilize independency to reduce binary calls. } 
In data-flow fuzzing, we try to invert at once multiple branches that do not depend on common bytes. This helps to reduce the number of executions by a factor proportional to the number of independent branches. 


\end{itemize}


\subsection{Old methods}
\ivica{Here goes what we took from others}

\begin{itemize}
\item AFL's showmap representation of edge coverage
\item GrayOne's branch inference based on branch values
\item RedQueen direct copy of bytes to obrain interval equations.
\item Score for testcases based on how many non-inverted branches and on uniqueness of branches.
\item Score branches based on how many non-inverted branches it has (but we do not sort, rather sample to score). 

\end{itemize}


\subsection{The whole fuzzer }
\ivica{ How everything is connected }

==> chapters/shiqi-problem.tex <==
% !TEX root = ../paper.tex

\section{Problems in Grey-box Fuzzing}

\input{figures/fuzzbench}

\prateek{It's not clear to me what you're trying to argue in the para below.}
Grey-box fuzzing is an effective technique for vulnerability detection and still an area of active research. Since 2011, a large quantity of grey-box fuzzing techniques (e.g., AFL~\cite{afl}, Honggfuzz~\cite{honggfuzz} and LibFuzzer~\cite{libfuzzer}) have been proposed by researchers every year. However, according to the evaluation reports generated by a free third-party service FuzzBench~\cite{fuzzbench}, none of the fuzzers significantly outperforms all the other fuzzers. Figure~\ref{fig:fuzzbench} shows the average rank of $13$ fuzzers reported by FuzzBench which are evaluated on $23$ real-world benchmarks.~\footnote{FuzzBench runs large-scale experiments on various fuzzers every few days and generates a report for comparison. In this paper, we gathered $73$ completed reports from FuzzBench and re-computed the average rank of $13$ out of $261$ fuzzers on $23$ out of $25$ benchmarks. 
We ruled out $2$ benchmarks on which more than $90\%$ of fuzzers do not evaluate and $248$ fuzzers which do not completely evaluate on these $23$ benchmarks.} The set of fuzzers that are connected with bold lines are not significantly different from each other. It is noteable that the coverage difference between these fuzzers is almost neglectable and no fuzzer consistently outperforms other fuzzers on all the evaluated benchmarks. 

\label{sec:problem}

\prateek{Why is dependency info / taint++ helpful for fuzzing to begin with?}

\prateek{Why is \textbf{dynamic selection of strategies} supposed to be useful, conceptually at least?
Right now you have an "argument by analogy" to SAT/SMT. Is this the way you want to keep it?}

\begin{enumerate}

\item Problem of inferring dependency on bytes when input is large (current state of the art is too slow). 

\item Problem of fuzzing strategies. Some strategies are very (in)efficient for some binaries.; hypothesize that universal fuzzing may not be possible, solution may be more similar to SAT solvers (where combination of strategies is more appropriate than a single principle). There are many choices that need to be made at each step of fuzzing. So, it makes sense to make available many options and then optimize the choice selection. 

\item Insufficient use of all information available to gray-boxes (everything up to SMT/SAT solvers). Can use better coverage, deploy better instrumentation, infer and use more data from the binary. 


\end{enumerate}

We address 1) in Sect~\ref{sec:inference} (propose new fast taint inference), 2) in Sect~\ref{sec:learning} (solution based on multi-armed bandits), and 3) in Sect.~\ref{sec:minor} (propose several improvements).


==> figures/fuzzbench.tex <==
\begin{figure}[t]
\centering
\resizebox{0.5\textwidth}{!}{%
\includegraphics[width=\linewidth]{figures/images/critical_difference_plot}
}
\caption{Average rank of $13$ fuzzers reported by FuzzBench which are evaluated on $23$ benchmarks. FuzzBench executes each fuzzer multiple times on each benchmark and calculates the median region coverage for ranking. The set of fuzzers that are connected with bold lines are not significantly different from each other.}
\label{fig:fuzzbench}
\end{figure}

==> figures/images/fuzzbench.tex <==
\begin{figure}[t]
\centering
\resizebox{0.5\textwidth}{!}{%
\includegraphics[width=\linewidth]{figures/images/critical_difference_plot}
}
\caption{Average rank of $13$ fuzzers reported by FuzzBench which are evaluated on $23$ benchmarks. FuzzBench executes each fuzzer multiple times on each benchmark and calculates the median region coverage for ranking. The set of fuzzers that are connected with bold lines are not significantly different from each other.}
\label{fig:fuzzbench}
\end{figure}
